Systematic Literature Review of AI-enabled Spectrum Management in 6G and Future Networks

Artificial Intelligence (AI) has advanced significantly in various domains like healthcare, finance, and cybersecurity, with successes such as DeepMind's medical imaging and Tesla's autonomous vehicles. As telecommunications transition from 5G to 6G, integrating AI is crucial for complex demands like data processing, network optimization, and security. Despite ongoing research, there's a gap in consolidating AI-enabled Spectrum Management (AISM) advancements. Traditional spectrum management methods are inadequate for 6G due to its dynamic and complex demands, making AI essential for spectrum optimization, security, and network efficiency. This study aims to address this gap by: (i) Conducting a systematic review of AISM methodologies, focusing on learning models, data handling techniques, and performance metrics. (ii) Examining security and privacy concerns related to AI and traditional network threats within AISM contexts. Using the Systematic Literature Review (SLR) methodology, we meticulously analyzed 110 primary studies to: (a) Identify AI's utility in spectrum management. (b) Develop a taxonomy of AI approaches. (c) Classify datasets and performance metrics used. (d) Detail security and privacy threats and countermeasures. Our findings reveal challenges such as under-explored AI usage in critical AISM systems, computational resource demands, transparency issues, the need for real-world datasets, imbalances in security and privacy research, and the absence of testbeds, benchmarks, and security analysis tools. Addressing these challenges is vital for maximizing AI's potential in advancing 6G technology.

==> sections/relatedwork.tex <==
\section{Related Work} \bushra{Working on it}
Numerous recent surveys have extensively examined the role of AI in 6G and future generation networks. However, the majority of these studies \citep{husen2022survey,wang2023road,sheth2020taxonomy, zhang20196g,shen2023five} primarily concentrated on application of AI  wider usage in 6G wireless communication . 
Nevertheless, the existing literature lacks comprehensive discussions on AI strategies for spectrum management in 6G and future generation networks. In Table \ref{comparison}, we present a comparative analysis of our Systematic Literature Review (SLR) and previous studies. Notably, many surveys only addressed , as evidenced by works such as [28], [230], [39], [10], [162], and [3]. Conversely, certain survey papers \citep{} made an effort to delve into attacks on board AI-enabled wireless and mobile computing approaches but failed to encompass all aspects of AI-enabled spectrum management 

\citep{sheth2020taxonomy} In this paper, a thorough survey is conducted on the integration of Artificial Intelligence (AI) in 6G communication technology, showcasing its potential across various future applications. The survey covers some aspect of Dynamic Spectrum Allocation, spectrum sensing and RF configuration. However, its not focused on AI for Spectrum Management in 6G. 


\citep{adesina2022adversarial} provides a thorough examination of recent research endeavors concentrating on Adversarial Machine Learning (AML) within the realm of wireless communications, taking into consideration the distinctive characteristics inherent in wireless systems. Initially, the document delves into the background of AML attacks on deep neural networks, offering an extensive taxonomy of AML attack types. The text proceeds to elucidate diverse methods for generating adversarial examples and delineates various attack mechanisms. Furthermore, a comprehensive survey is conducted, encompassing existing research on AML attacks concerning diverse issues in wireless communication, along with the corresponding defensive mechanisms within the wireless domain. Lastly, the paper addresses contemporary research trends and anticipates the future landscape of AML within next-generation wireless communications, highlighting both emerging attacks and evolving defense techniques.
It covers some studies related to spectrum sensing and resource allocation at network layer (network slicing). It focus on the adversarial attacks on these systems. 

\citep{liu2021adversarial} The survey article systematically maps and reviews the state-of-the-art in Adversarial Machine Learning (AML) as applied to wireless and mobile systems. It covers AML approaches from the physical layer to the application layer, focusing on the generation and detection of adversarial samples. These samples are created using techniques like Generative Adversarial Networks (GANs) and Fast Gradient Sign Method (FGSM). Detection methods involve adversarial models as classifiers or machine learning classifiers with knowledge on identifying such samples. The article provides high-level overviews of each approach, emphasizing their impact on solving challenges in wireless and mobile settings. Additionally, it delves into the configuration (CFG) impact and discusses open issues, challenges, and research opportunities, offering valuable insights for AI-driven wireless and mobile networking researchers and developers.
Not focused on spectrum management, does not provide a hositic view of the state-of-the-art also, the scope it more broader than detailed focus on ML.
\citep{wang2023adversarial}
the survey aims to offer a comprehensive overview of recent advancements in adversarial attacks and defenses, specifically within the context of DNN-based classification models in communication applications. The visual presentation, thorough evaluation, and emphasis on challenges contribute to the broader understanding of this evolving and critical research area.
Don't focus on spectrum management, or 6G .  he survey offers a comprehensive examination of the recent developments in adversarial attacks and defenses within the field of machine learning (ML) and artificial intelligence (AI), with a particular focus on the past 24 months. As ML and AI applications continue to expand across various domains, the security and robustness of models have become paramount. The survey reviews over 220 research papers from reputable sources and top-tier conferences, concentrating on attacks and defenses relevant to ML or deep neural network (DNN)-based models in communication and networking. It provides a detailed classification of recent adversarial attack methods and state-of-the-art defense techniques, categorizing them into counter-attack detection and robustness enhancement. The evaluation of existing works includes a nuanced analysis of strengths and limitations, while also exploring new attack avenues and acknowledging the emergence of physical-world adversarial attacks. The hierarchical classification of defense methods addresses challenges and aims to inform and inspire further research and innovation in this rapidly evolving domain, ensuring the research community and security practitioners stay well-informed about the latest developments. Focus on adversarial attacks only. It cover some attacks on spectrum sensing, monitoring and channel fading. 


\citep{jasim2021survey} the survey aims to fill a gap in existing literature by providing a detailed examination of spectrum management tailored to the unique characteristics of UAV networks. It covers regulatory aspects, deployment scenarios, management tools, and potential solutions, ultimately contributing to the understanding and development of efficient and safe UAV communication systems. Does not focus on Ml approaches, does not focus of over spectrum management in 6G but limited to spectrum management in UAV. 


\citep{du2020machine} A comprehensive guide to the potential of machine learning in the context of 6G wireless networks. It discusses the expected capacities of 6G networks, including ultrabroadband, ultramassive access, ultrareliability, and low latency. The paper also explores the challenges posed by the complex architecture of 6G networks and how machine learning can help with channel estimation, spectrum management, and network orchestration and management. Additionally, the paper highlights the importance of data privacy and security in the implementation of machine learning algorithms in 6G networks.  It provides a detailed and informative overview of the potential of machine learning in the context of 6G wireless networks.

\citep{husen2022survey} in essence, the study explores the intersection of Machine Learning and Future Intelligent Networks, highlighting the need for advanced ML techniques that can address the challenges of a heterogeneous, multi-domain network environment while promoting holistic decision-making and problem-solving. Massive data traffic rise in FIN requires intelligent
spectrum management techniques for improving spectrum utilization. Intelligent spectrum man- agement has been extensively addressed using SL and UL approaches in the literature. Spectrum prediction has also become a vital research area due to its wide applications in cognitive radios. It includes spectrum sensing, mobility, dynamic spectrum access, and intelligent topology control [197]. As canbeseeninTable 10, in the literature there are several RL-based techniques for dy- namic spectrum [198], spectrum efficiency [199, 200], spectrum sharing [201], spectrum allocation [202], and spectrum prediction [203].
% Furthermore, they were only limited to elaborating on the use of DL models in a single platform such as Android or Windows. For instance, the survey conducted in [237] was only focused on DL techniques for malware detection in Android. Nevertheless, topics such as frameworks for building DL models, network optimization, activation, and regularization techniques were not covered. Another example is the survey conducted by Gibert et al. [74], which explored DL techniques for malware detection in the Windows platform. However, their work is also limited and did not cover recent DL technologies such as optimization and activation techniques as well as frameworks for implementing DL models. It is also worth noting that they did not also explore malware detection in the Linux and Android platforms. Overall, the previous surveys highlighted in Table 1 have many limitations which we believe are crucial research gaps in the literature. Therefore, this work aims at presenting a detailed and comprehensive survey of recent DL technologies and their applications for malware detection in Windows, Linux, and Android platforms. These platforms were chosen as they are currently the most popular, targeted, and infected by malware attacks, among others. The following are our contributions to the literature.
\textbf{Novelty} 
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
    \textbf{Surveys} &Year& Coverage Duration & Spectrum Management & AI & Datasets & Performance Measures & Learning Algorithms& 5G+ & Physical Layer & Security and Privacy & Adversarial Security and Privacy \\ 
\end{tabular}%
}
\caption{Summary of Research Papers on AI in Spectrum Management}
\label{comparison}
\end{table}

% \begin{itemize}
%     \item Adversarial ML for RF 
% \end{itemize}
% \begin{table}[H]
%     \centering
%     \resizebox{\textwidth}{!}{%
%         \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%             \hline
%             \textbf{Paper ID} & \textbf{Study} & \textbf{Read By} & \textbf{Year} & \textbf{Venue Type} & \textbf{Venue} & \textbf{Summary} & \textbf{Spectrum Management Topics Covered} & \textbf{Spectrum Management Topics} & \textbf{Comments} \\
%             \hline
%             Paper 1 & A Survey on Requirements... & Bushra Sabir & 2022 & Journal & ACM Computing Survey & In essence, the study explores... & Application of ML in Network Slicing... & dynamic spectrum [198], spectrum efficiency... & Covers overall application of AI in 6G... \\
%             \hline
%             Paper 19 & On the Road to 6G: Visions... & Bushra Sabir & 2023 & Journal & IEEE survey of communications and tutorials & Fifth generation (5G) mobile communication... & Spectrum Resource Challenges: The need to... & Cognitive Radio (CR), Symbiotic Radio (SR)... & Comparison between 5G and 6G in terms of... \\
%             \hline
%             Paper 4 & A Comprehensive Survey of Spectrum... & Bushra Sabir & 2022 & Arxiv & Arxiv & The paper addresses the challenges... & Spectrum Sensing, Resource Allocation... & Artificial Intelligence, Coexistence Analysis... & \\
%             \hline
%             Paper 6 & MACHINE LEARNING FOR 6G WIRELESS... & David & 2020 & Magazine & IEEE VEHICULAR TECHNOLOGY MAGAZINE & A comprehensive guide to the potential... & AI/ML techniques for wireless networks... & channel estimation, spectrum management... & \\
%             \hline
%             Paper 7 & A taxonomy of AI techniques for... & David & 2020 & Journal & Computer Communication & The paper discusses the potential of 6G... & Discusses spectrum management in 6G networks... & Dynamic spectrum management, cognitive radio... & Vague on security topics \\
%             \hline
%             Paper 21 & Spectrum Management in the 6G Era... & Shuiqiao & 2020 & Conference & 6G Wireless Summit (6G SUMMIT) & The paper discusses the evolving landscape... & Discussion of various spectrum management... & Historical methods: administrative allocation... & Vague on security topics \\
%             \hline
                
%             \hline
            
%             \hline
%             Paper 5 & Five Facets of 6G: Research... & Bushra Sabir & 2023 & Journal & ACM Computing Survey & & & & \\
           
%              \hline
            
%             \hline
%         \end{tabular}%
%     }
%     \caption{Table caption goes here.}
%     \label{tab:mytable}
% \end{table}

==> sections/resultRQ2_Old.tex <==
%[Shuiqiao in-charge] If we have AI-based Spectrum management what are the challenges in it.
\section{RQ2: Security and Privacy Challenges of AI-enabled Spectrum management (AISM)}
\label{sec:securityandprivacy}
\bushra{Revision Required Throughly}


% \begin{tcolorbox}[
%     enhanced,
%     colback=white,
%     colframe=teal,
%     arc=0pt,
%     outer arc=0pt,
%     boxrule=0.8pt,
%     %borderline west={0.5mm}{-1mm}{teal},
%     sharp corners,
%     title={Summary and Insights},
% ] 
%   \begin{enumerate}
%       \item \textbf{Attacks on AI Models: }In this section, we delve into the various adversarial attacks targeting AI models in spectrum management, such as adversarial manipulations, backdoor threats, privacy disclosures, and data leakage. The discussion focuses on how these attacks can undermine the integrity and effectiveness of AI-driven spectrum management, highlighting the complexities these threats pose.
%       \item \textbf{Physical Layer Attacks: }This section examines physical layer attacks, including jamming, eavesdropping and spoofing, which pose significant threats to spectrum management. It explores the impact of these attacks on the stability and security of communication systems, demonstrating the need for effective countermeasures.
%       \item \textbf{Defensive Strategies for Spectrum Management: }In this section, we explore a range of defensive strategies deployed to safeguard AI systems in spectrum management. The focus is on developing robust AI models, implementing fingerprinting for authentication, and utilizing anomaly detection, among other measures. This discussion illuminates how these strategies fortify spectrum management systems against diverse cyber threats.
%   \end{enumerate}

% \end{tcolorbox}

% \begin{figure*}[h!]

% \centerline{\includegraphics[width=0.8\textwidth]{sections/Figures/RQ2.pdf}}
% \caption{The Security and Privacy challnges for AISM. }
% \label{fig:sec5_overview}
% \end{figure*}

% \begin{figure}[h!]

% \centerline{\includegraphics[width=0.8\textwidth]{sections/Figures/references_figure.pdf}}
% \caption{The Number of Studies.}
% \label{fig:num_reference}
% \end{figure}


%The integration of AI into spectrum management for 5G, 5G beyond, and the forthcoming 6G networks holds immense promise, offering dynamic and efficient allocation of wireless resources, enhanced performance, and improved user experiences. However, in addition to these remarkable benefits, a parallel landscape is rife with risks and challenges that require careful consideration. As wireless communication networks evolve to meet the demands of an increasingly connected world, they become more intricate and susceptible to a spectrum of adversarial threats. These threats span the gamut from traditional jamming attacks to sophisticated adversarial machine-learning tactics, including membership inference attacks, eavesdropping, and model poisoning. Therefore, ensuring the robustness, security, and privacy of AI-driven spectrum management systems is imperative, as any compromise in these domains can lead to service disruptions, data breaches, and network vulnerabilities. In this context, it is crucial to explore these risks comprehensively, as they cast a shadow over the potential benefits of AI in spectrum management, and to devise strategies for safeguarding the integrity and reliability of our wireless networks. 

In this section, we will dive into the risks, examine the  implications, and explore the proactive measures and defensive strategies necessary to mitigate the security and privacy challenges of AISM.
Figure \ref{fig:sec5_overview} offers a succinct summary of the security and privacy challenges, delineating them into AI Attacks with subcategories like adversarial, evasion, and poisoning threats; Physical Layer Attacks involving jamming, eavesdropping, and spoofing; and an array of Defensive Strategies tailored to mitigate these risks with robust AI models, authentication protocols, privacy-preserving methods, anomaly detection and anti-jamming. 
Figure \ref{fig:num_reference} shows the total number of references we have included in this section. 
%In the forthcoming sections, we will delve deeper into each subtopic presented in the summarized figure, exploring the nuances and intricacies that define the state-of-the-art in AISM security and privacy, and proposing solutions to fortify our systems against these evolving threats.


%\sha{Good place to introduce the Figure 5.1 and explain it high level.Then you go below to them one by one. Also for Robust AI Models in the figure - please change its location to top?}

% \begin{table}[h]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Type of Attack} & \textbf{Description} & \textbf{Reference} \\ \hline
% Adversarial Manipulations & Attacks aiming to mislead AI models & [1] \\ \hline
% Backdoor Threats & Hidden triggers in AI models altering behavior & [2] \\ \hline
% Privacy Disclosures & Unauthorized access to sensitive data & [3] \\ \hline
% Data Leakage & Inadvertent exposure of confidential information & [4] \\ \hline
% \end{tabular}
% \caption{AI Attacks in Spectrum Management}
% \label{tab:ai_attacks}
% \end{table}

\subsection{AI Attacks}
%In the intricate battlefield of AISM, our immediate focus narrows down to two predominant forms of AI attacks that stand as formidable threats to security and privacy: adversarial and privacy attacks. As we venture into this discussion, it is crucial to acknowledge the paradox that AI models present; while they are instrumental in advancing spectrum management, they also introduce significant risks due to their non-explainable, 'black-box' nature and inherent vulnerabilities. Adversarial attacks, including the insidious data poisoning and cunning adversarial example techniques, directly target the core functioning of AI models, aiming to manipulate or mislead. Privacy attacks, on the other hand, stealthily undermine the confidentiality of data, posing a grave risk to the integrity of spectrum management systems. 
% In this subsection, we will scrutinize the likes of evasion attack, data poisoning, backdoor attacks, adversarial example attack, as well as the privacy disclosure attacks such as data leakage and membership attacks. 
%This high-level overview will serve to underscore the urgency and necessity of developing more resilient and transparent AI systems in the spectrum management landscape, where the stakes are as high as the rewards.

\subsubsection{Adversarial Attacks}

Adversarial attacks on AI models in spectrum management represent a critical vulnerability, as they are designed to exploit the models' weaknesses and compromise the entire spectrum management system.
%These attacks are multifaceted and sophisticated, each with its own methodology and impact. Our examination will dissect these attacks into their respective categories to better understand and develop strategies to mitigate their effects.

\paragraph{Evasion}
\bushra{Added missing paper if extras will be included in methodology, combined evasion and adversarial examples, the purpose of both is same}
In \citep{flowers2019evaluating} 
the authors delves into the susceptibility of Radio Frequency Machine Learning (RFML) systems, especially in Automatic Modulation Classification (AMC), to adversarial evasion attacks. These attacks manipulate input signals to mislead classifiers, posing significant security risks for RFML applications in spectrum sensing and dynamic spectrum access. The study distinguishes between digital and over-the-air attacks, emphasizing the complexity of defending RFML in real-world scenarios. It introduces a novel evaluation method based on bit error rate, highlighting RFML's vulnerabilities yet suggesting that inherent signal processing challenges could naturally limit these attacks' success. This research underscores the urgent need for developing robust defenses for RFML systems in the context of wireless communications security.

Another study [S33]. reveals deep learning-based wireless signal classifiers' vulnerability to adversarial attacks, posing a significant threat to spectrum sensing reliability. Initial attacks without channel consideration fail, but channel-aware and broadcast adversarial strategies significantly compromise classifier accuracy. The research highlights the critical security risks in using deep learning for signal classification and proposes a defense mechanism, randomized smoothing, to enhance resilience against such attacks. This underscores the urgent need for advanced defense methods to protect spectrum sensing from adversarial threats.
Another work \citep{bahramali2021robust}  work examines the vulnerability of Deep Neural Networks (DNNs) used in wireless communication systems to adversarial attacks, which can significantly compromise the security and reliability of these systems. By designing robust adversarial examples that adhere to the unique constraints of wireless systems, such as being undetectable from natural noise and robust against removal, the study demonstrates that DNN-based wireless systems, including those used for channel estimation, signal decoding, and modulation recognition, are highly susceptible to such attacks. Despite defensive efforts, the research reveals that these systems remain vulnerable, raising concerns about the reliance on DNNs for critical tasks in wireless communication. The findings are supported by comprehensive evaluations across various DNN-based wireless applications, showing the effectiveness of the adversarial attacks in degrading system performance and highlighting the need for more resilient defense mechanisms.
\citep{mitchell2023exploring}, focus shifts towards understanding and mitigating evasion attacks against spectrum sensing in RF transmitter localization. Evasion attacks, wherein adversaries manipulate sensor data to mislead the localization process, pose a significant challenge. By employing a Convolutional Neural Network (CNN) trained on real-world data, the research assesses the vulnerability of the localization system to such deceptive tactics. The study systematically explores the effectiveness of adversarial training and statistical outlier detection as countermeasures. Findings reveal that these strategies significantly enhance the system's resilience by improving its ability to identify and neutralize manipulated inputs, thereby preserving the accuracy of transmitter localization despite adversarial attempts to evade detection. This insight is crucial for developing more secure and reliable machine learning-based systems in the context of mobile computing and communications, where the integrity of sensor data is paramount.
%Evasion attacks represent a sophisticated form of cyber assault, where adversaries craft malicious inputs to evade AI detection during the inference phase. In the context of spectrum management, this could manifest as unauthorized bandwidth usage or circumvention of regulatory checks. These attacks exploit the decision boundaries of AI models, manipulating signals to effectively become 'invisible' to AI monitoring systems, thus posing a serious threat to the fair and lawful allocation of spectrum resources.

% Evasion attacks aim to mislead or disrupt the mechanism. These attacks focus on degrading system performance or disrupting availability by targeting control frames crucial for beamforming. Specifically, they attack control frames, potentially causing a denial-of-service (DoS) impact on both the transport layer and application layer. 
% Techniques such as low air time jamming and "off-target jamming" are used to discreetly target the system, significantly reducing TCP throughput or causing outages by attacking vital setup messages in transport and application layers.
% Addressing evasion attacks in spectrum management, particularly with the growth of high-speed network mobile applications in the IIoT, is both complex and critical. 
% The widespread occurrence of Android malware, amplified by the complexity of IIoT applications, poses a significant security threat~\citep{rafiq2022mitigating}. This challenge is further heightened by the vulnerability of federated learning (FL) systems, commonly used for radio signal classification, to model poisoning attacks that can severely compromise the integrity of global classifiers, undermining network reliability~\citep{rafiq2022mitigating}.
% In response, there is an increasing focus on developing sophisticated AI and machine learning (ML) algorithms capable of proactively identifying and countering evasion attacks. This involves not only enhancing the security of existing systems but also creating new models that can adapt to the changing strategies of attackers.


% In response to these multifaceted challenges, several innovative defense strategies have been developed. One approach involves the use of subset feature selection and ensemble-based learning. These methodologies are designed to detect and evade fabricated attacks within the IIoT environment, enhancing the resilience of systems against sophisticated malware~\citep{wang2023mitigating}. Another notable development is the Underlying Server Defense of Federated Learning (USD-FL), a framework specifically tailored to safeguard FL-based signal classifiers. This defense mechanism addresses the vulnerabilities inherent in FL systems, offering a more robust defense against model poisoning~\citep{wang2023mitigating}.

% Moreover, the increased reliance on AI-based semantic segmentation models in cellular networks for spectrum sensing has exposed new vulnerabilities. Recent vulnerability analyses of these AI-driven approaches have underscored the pressing need for effective mitigation methods. These methods are crucial for reducing the system's exposure to adversarial attacks, which can otherwise exploit these weaknesses to disrupt network operations~\citep{catak2022mitigating}.



% \begin{table}[h]
% \centering
% \begin{tabular}{|p{0.3\linewidth}|p{0.7\linewidth}|}
% \hline
% \textbf{Issue/Technology} & \textbf{Challenges/Defense Strategies} \\
% \hline
% Evasion attacks in spectrum management & Detection and counteraction of evasion attacks is critical in the IIoT context, with challenges intensified by the proliferation of Android malware and the susceptibility of FL systems to model poisoning, compromising the training of global classifiers~\citep{rafiq2022mitigating}. \\
% \hline
% Defense strategies in IIoT & Use of subset feature selection and ensemble-based learning for detecting and evading fabricated attacks, enhancing system resilience against sophisticated malware. Implementation of USD-FL framework to safeguard FL-based signal classifiers against model poisoning~\citep{wang2023mitigating}. \\
% \hline
% AI-based semantic segmentation in cellular networks & The reliance on AI models for spectrum sensing has exposed vulnerabilities to adversarial attacks. Vulnerability analyses highlight the need for effective mitigation methods to protect network operations~\citep{catak2022mitigating}. \\
% \hline
% \end{tabular}
% \caption{Challenges and Defense Strategies of Evasion Attacks in Spectrum Management for IIoT}
% \label{tab:spectrum_management_challenges}
% \end{table}


% \textcolor{black}{Shuiqiao: we need some references here. } done by NW

\paragraph{Data Poisoning}

\bushra{4 papers 3 in our extracted data, one additional was added my me. However, paper that was cited in it shi2018spectrum doesn't fullfil our inclusion and exclusion criteria}
Data poisoning attacks are aimed at corrupting the training data on which AI models in spectrum management rely. 

In the specific context of spectrum management, data poisoning attacks represent a sophisticated form of cyber warfare. Adversaries execute these attacks by deliberately manipulating the spectrum sensing data of a transmitter, with the aim of leading it to make incorrect decisions regarding its transmissions. These attacks are typically conducted by transmitting signals during the transmitter's spectrum sensing periods, causing a false perception of the channel status as 'busy' rather than 'idle'. Such attacks are energy-efficient and challenging to detect but can significantly reduce the transmitter's throughput. This results in substantial disruptions in communication and data flow, posing a serious threat to the system's integrity [S31, S32, S18]  ~\citep{zhang2022poison}.

 In [S31], this paper introduces a Learning-Evaluation-Beating (LEB) attack framework. This framework, based on adversarial machine learning, is designed to launch attacks against cooperative spectrum sensing.
To counter the LEB attack, the paper introduces a non-invasive defense method called influence-limiting defense, which can coexist with existing defenses and reduces the overall disruption ratio of the LEB attack by up to 80\%.

% What papers have done it?
\paragraph{Backdoor Attacks}

%Add 



Backdoor attacks in AI models present a covert and serious threat to spectrum management. These attacks involve embedding hidden triggers that, when activated, alter the model's behavior to the attacker's advantage, often remaining undetected under normal operating conditions. 

In the context of spectrum management, such attacks could enable unauthorized entities to access or prioritize spectrum, particularly during congested periods. The insidious nature of backdoor attacks lies in their ability to make the AI model perform normally until the hidden trigger is activated, posing significant detection challenges.

\bushra{[Papers mentioned in this paragraph are Not Related to Spectrum Management, can be a discussion pointed]
\textit{Types of Backdoor Attacks:} 
\begin{itemize}
    \item \textbf{Training Dataset Manipulation:} A common type involves inserting triggers into the training dataset of a neural network. These triggers are designed to modify the network model's behavior under specific conditions, leading to undesirable actions or outcomes~\citep{hadi2022types}. 
    \item \textbf{Spoofing and Mimicry:} Another form entails spoofing or mimicry within wireless networks. Adversaries may inject false nodes, fabricate identities, or engage in IP spoofing, disrupting network operations by creating false perceptions of network activities or statuses~\citep{abad2022poster}.
    \item \textbf{Semantic Communication Attacks:} Backdoor attacks also target semantic communications, where communication is based on transmitted data's meaning. Triggers in training samples can subtly alter the conveyed meaning, leading to misinterpretation or message manipulation, causing communication disruptions~\citep{raguvaran2014spoofing}.
\end{itemize}
Backdoor attacks in wireless communications and spectrum management take various forms, each exploiting different aspects of network operations. From altering training datasets to spoofing network identities and manipulating semantic communications, these attacks represent a significant security challenge, requiring sophisticated detection and mitigation strategies.
}

\bushra{This paper can be added for keeping the taxonomy intact \citep{zhang2022backdoor}}




% \paragraph{Backdoor}

% Backdoor attacks are a surreptitious method of embedding a hidden trigger in an AI model. When activated, the model's behavior is altered to the attacker's benefit. For spectrum management, this could result in certain entities gaining unauthorized access to spectrum or priority during congested periods. This form of attack is particularly insidious because the model may perform normally under regular conditions and only behave maliciously when the backdoor is triggered, making detection exceptionally challenging.

% Backdoor attacks in wireless communications represent a significant security threat, taking various forms and exploiting different aspects of network operations. One common type of backdoor attack involves the insertion of triggers into the training dataset of a neural network. These triggers are designed to alter the behavior of the network model under specific conditions, leading to malicious actions or outcomes when those conditions are met~\citep{hadi2022types}.
% Another form of backdoor attack is the spoofing or mimicry of information within wireless networks. In these scenarios, adversaries can inject false nodes, fabricate identities, or engage in IP spoofing to mislead or disrupt network operations. This type of attack is particularly insidious as it can create a false perception of network activities or statuses, leading to incorrect decisions or responses from the network~\citep{abad2022poster}.
% Additionally, backdoor attacks can target semantic communications, a method where communication is based on the meaning of the transmitted data rather than its syntactic representation. In these attacks, triggers are added to training samples to subtly alter the meaning conveyed to the receiver. This can lead to misinterpretation or manipulation of the message, causing significant disruptions in communication~\citep{raguvaran2014spoofing}.




% \textcolor{black}{Shuiqiao: we need some references here. } done by NW


\subsubsection{Privacy Disclosure}

As we continue to navigate the complex terrain of AI in spectrum management, we must turn our vigilant gaze to the specific challenges posed by privacy attacks. 
These insidious intrusions target the very lifeblood of AI systems—the data. Within this scope, we encounter two particularly pernicious threats: data leakage attacks and membership inference attacks. 



\paragraph{Data Leakage}
[S23,
,S33
,S45] Data leakage and membership inference attacks in our extracted data.
\bushra{I found no paper related to our SLR in this subsection}
Data leakage in AISM is a critical domain, highlighting the risk of sensitive information inadvertently being exposed through the AI models themselves. 
In spectrum management, the implications are particularly severe, as the leaked data may include proprietary system configurations, user activity logs, or even national security-related information. This type of attack can originate from various points in the AI lifecycle, from initial data collection to model deployment, and may result from either direct attacks on the database or inadvertent leaks due to flaws in model design. 
%As AI systems become increasingly integrated into the spectrum allocation process, the need to establish robust protocols and defensive mechanisms to prevent data leakage becomes imperative. This section will explore the various avenues through which data leakage can occur in spectrum management and the best practices for safeguarding against such vulnerabilities.

\begin{itemize}
    % \item \textbf{Regulatory and Legal Consequences}:The complexity of data sharing between different countries and areas introduces additional challenges. Different jurisdictions have varying data protection regulations, such as the General Data Protection Regulation (GDPR)~\citep{regulation2018general} in the European Union or the Health Insurance Portability and Accountability Act (HIPAA)~\citep{edemekong2018health} in the United States. This requires a comprehensive understanding of international data protection standards and the implementation of versatile data protection strategies that can adapt to various legal requirements.
    
    \item \textbf{Inadequate Security Protocols}: Weaknesses in security protocols pose a significant risk in AISM, potentially leading to unauthorized access to sensitive spectrum allocation data. To address this vulnerability, private blockchain-based security schemes have been devised. These schemes aim to enhance the security of spectrum allocation processes by ensuring that access is granted exclusively to authorized users. The use of blockchain technology in this context offers increased security and transparency, making it more difficult for unauthorized entities to manipulate or access the data~\citep{br2023blockchain}. \bushra{Not suitable, not fullfilling inclusion and exclusion criteria. Can be a discussion point}
    
    In addition to these measures,
    there has been an increased focus on the vulnerability of spectrum allocation in cognitive radio networks. Such networks are susceptible to specific types of attacks, like the Channel Ecto-Parasite Attack (CEPA). This attack exploits weaknesses in spectrum management protocols, potentially leading to unauthorized access or disruption of the network. The exposure of this vulnerability underscores the urgent need for more robust and sophisticated security measures in spectrum management~\citep{cheng2020lightweight}. \bushra{The reference is not in our extracted paper list but fulfills the criteria }
    
    \item \textbf{Allocation of spectrum bands}: The process of allocating spectrum bands to different services or providers carries the risk of data leakage, a concern that has been highlighted in recent studies~\citep{papadimitriou2010data}.
    This risk is particularly pronounced in the realm of cognitive radio networks, where collaborative sensing among multiple service providers introduces significant privacy challenges~\citep{li2010spectrum}.
    In these networks, the sharing of sensing data as part of collaborative schemes can inadvertently provide opportunities for malicious entities. These entities could exploit the shared data to geolocate secondary users, thereby compromising their privacy and potentially leading to further security breaches~\citep{chavan2013data}. \bushra{Not meeting our criteria}
\end{itemize}

\textbf{Regulatory and legal consequences}  play a critical role in preventing data leakage, especially in the context of data sharing across different countries and regions. The complexity of data sharing between different countries and areas introduces additional challenges. Different jurisdictions have varying data protection regulations, such as the General Data Protection Regulation (GDPR)~\citep{regulation2018general} in the European Union or the Health Insurance Portability and Accountability Act (HIPAA)~\citep{edemekong2018health} in the United States. This requires a comprehensive understanding of international data protection standards and the implementation of versatile data protection strategies that can adapt to various legal requirements.


% \textcolor{black}{Shuiqiao: we need some references here. } done by NW

% \paragraph{Membership Inference} 
% Membership inference attacks present a unique challenge 
% in the realm of AI-enabled spectrum management by threatening the anonymity and privacy of the data subjects. These attacks specifically target the models to determine if data from particular users or devices was included in the model's training dataset. For spectrum management, this could lead to the disclosure of sensitive user behaviors, such as the time and frequency of spectrum use, which could be exploited for competitive advantage or malicious intent. The sophistication of these attacks is a testament to the vulnerabilities inherent in the AI models used for spectrum management, especially when handling vast amounts of confidential data. In this section, we will dissect the methodology of membership inference attacks, their potential impact on spectrum management, and the strategies that can be employed to detect and mitigate such privacy intrusions.

% working on this part now~
% no findings...

%\textcolor{black}{Shuiqiao: we need some references here. cannot find any. suggest remove this section}

% \begin{table}[h]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Type of Attack} & \textbf{Description} & \textbf{Reference} \\ \hline
% Jamming & Deliberate interference disrupting communications & [5] \\ \hline
% Eavesdropping & Unauthorized interception of private communications & [6] \\ \hline
% Spoofing & Falsifying signals or data to deceive systems & [7] \\ \hline
% \end{tabular}
% \caption{Physical Layer Attacks in Spectrum Management}
% \label{tab:physical_layer_attacks}
% \end{table}


\subsection{Physical Layer Attacks}
%\textcolor{green}{Shangqi: I think this section is more about defence strategy on Physical Layer Attacks, do we need to consider the title again?}
%\sha{We need some references to the below text. Also, it seems way toward eveasdroping. How about Jamming and Spoofing??}
%\sha{We need to keep only few papers relvent to Physical layer security somehow. We move the others to Jamming, evesedroping and Spoofing. Also, the paragraphs now not connected. We need some entry sentences at the start for the review to have an idea what's coming. Then try to connect the papers.}
%\subsection{Physical Layer Security}
The physical layer of spectrum management serves as the foundation for communication systems, and as such, it is frequently the target of malicious attacks that can have devastating effects on the integrity and availability of wireless communications. %Physical Layer Security (PLS) is a fundamental concept in information theory and network security, employing the inherent physical characteristics of the communication channel for data protection. Unlike conventional cryptographic techniques that rely on mathematical algorithms, PLS harnesses the attributes of the physical medium itself. PLS emerges as a promising approach to enhance the security capabilities of B5G networks, which are anticipated to accommodate the increasing demands of users. Safeguarding against eavesdroppers seeking to intercept and exploit valuable information in such high-traffic settings is as formidable a task as excluding them from the network. 
This section will delve into the primary types of physical layer attacks that jeopardize AISM systems: jamming, spoofing, and eavesdropping.
In the following sections, we will dive into the details about the different types of physical layer attacks in spectrum management.
% Some key aspects of PLS are listed below:

% \begin{itemize}
%     \item \textbf{Channel Characteristics}: PLS exploits properties such as signal strength, noise levels, fading, and other inherent traits of the communication channel. For instance, it may capitalize on the fact that an eavesdropper's signal is weaker than the legitimate receiver's, often due to factors like distance or obstacles.
%     \item \textbf{Secrecy Capacity}: This metric serves as a cornerstone in PLS. It quantifies the maximum amount of information that can be securely transmitted over a channel, factoring in both the legitimate receiver's and eavesdropper's channels.
%     \item \textbf{Wireless Environment}: PLS finds particular relevance in wireless communication scenarios, where detecting eavesdropping can be more challenging compared to wired communication.
%     \item \textbf{Eavesdropper Mitigation}: PLS aims to minimize the information accessible to potential eavesdroppers. This objective can be achieved by designing the communication system in a manner that makes it harder for unauthorized parties to intercept and decode transmitted information.
%     \item \textbf{Keyless Security}: In contrast to traditional cryptographic systems, which necessitate shared keys, PLS does not rely on pre-shared secret keys between communicating parties. Instead, it exploits the characteristics of the physical medium.
    
% \end{itemize}

% However, PLS encounters challenges such as the requirement for precise channel state information, susceptibility to noise and interference, and the necessity for advanced signal processing techniques.







% Additionally, a paper by Chen et al. \citep{chen2021impact} explores the impact of residual hardware impairment (RHI) on the secrecy performance of RIS-assisted NOMA networks. The study scrutinizes the factors influencing secrecy outage probability and demonstrates that RHI can detrimentally affect the system's secrecy outage performance. The severity of this impact hinges on the transmit Signal-to-Noise Ratio (SNR) and target data rate. The paper also illustrates that RIS-assisted NOMA enhances secrecy performance in comparison to traditional NOMA. However, there is no mention of the utilization of AI in the research or its application in the discussed system.

% NAN
%\subsubsection{Physical layer security using Beamforming}





\subsubsection{Jamming Attack}

Jamming attacks are a form of deliberate interference that disrupt the normal functioning of communications by overwhelming the spectrum with noise or unwanted signals. This can lead to a denial of service for legitimate users, severely impacting the reliability of wireless communications.
In [S27], a strategy is proposed to detect and mitigate resource selection jamming attacks in NR-V2X distributed mode. The scheme effectively reduces packet dropping-based attacks and improves packet reception ratio. The attackers aim to disrupt communication by causing consecutive collisions to the victim, rendering it undetected on the road. 
%They select resources and schedule beacon messages to achieve this objective.
% The defense strategies presented in the paper encompass: a) \textit{Attacker Mitigation}: Victim vehicles can select a new Radio Resource Unit (RU) after each beacon transmission, rendering the attack futile. Another option involves making the resource selection adaptive.
% b)\textit{ Attack Detection:} A feedback mechanism is introduced for detecting attacks. Victims can identify the attacker by consulting the table of last received beacons, with feedback provided by nearby vehicles.
% c) \textit{Attack Mitigation}: Upon detecting an attack, the victim vehicle adjusts its resource reservation period using a fuzzy inference system (FIS) to determine the duration for employing the next selected RU. The FIS, a decision-making algorithm, establishes the RC value based on inputs, namely, the Number of Dropped Packets and the Channel Busy Ratio (CBR).
In [S34], deep learning-driven physical layer security is proposed. The paper explores the application of deep learning for resource allocation in a Simultaneously Wireless Information and Power Transfer (SWIPT) network. The goal is to maximize the minimum achievable secrecy rate for the legitimate user while satisfying the energy harvesting requirements of the energy receivers (ERs). \bushra{Additional References can be added, jere2023bayesian
sharma2023secrecy
feng2023securing}
%Traditional resource allocation problems are typically addressed through convex optimization approaches, which can be time-consuming. To address the need for ultra-low latency and achieve physical layer security in SWIPT systems, 
%The authors develop a deep neural network (DNN) based approach, significantly reducing computational time and complexity. 
%The DNN is trained through repeated simulations to determine weights and biases, and feed-forward calculations are employed to optimize power allocations in the SWIPT network. Numerical results demonstrate the effectiveness of the proposed DNN-based approach in achieving near-optimal secrecy rate performances compared to convex optimization approaches.
%PLS using beamforming techniques for 5G and beyond networks. 
%In another work \citep{sharma2022physical}, the authors discuss various PLS applications that use beamforming based techniques along with their potential shortcomings and research challenges in detail. It also addresses various PLS issues and research questions related to 5G and beyond networks' security using beamforming based techniques. The paper compares the most related surveys with the proposed survey using the research questions summarized in Table 2~\citep{sharma2022physical} described in detail,he findings of previous PLS research surveys in comparison to the proposed one by highlighting the major differences. The paper also discusses other PLS approaches that can be combined with beamforming to further improve the security of 5G and beyond, such as Artificial Noise (AN) injection, Cooperative Jamming (CJ), Secure Channel Coding (CC) techniques. Finally, the paper provides a taxonomy of the manuscript and possible future directions for research in this field.

\subsubsection{Eavesdropping Attack}

%\sha{Potential section to reduce. Maybe summarise into 1 pager and have a table for the several factors where you have the factor and few columns as brief}
Eavesdropping represents a more passive but equally dangerous threat, where unauthorized entities intercept confidential communications. In spectrum management, eavesdropping can result in the loss of sensitive information, violating user privacy and potentially compromising strategic operations.

%\sha{This is eveasdropiing paper. Might go to relevant eavesdropping subsection?}
The study [S53] analyzes the effectiveness of artificial noise (AN) in enhancing the security of physical layer (PHY) transmissions. PHY security leverages the unique properties of the wireless medium to provide security and make it challenging for attackers to detect information.
%Approaches such as full-duplex communication and artificial noise are employed to thwart eavesdropping attacks and provide immunity. Techniques such as the generation of secure probability maps, the channel correlation map, and the creation of secure regions are utilised to enhance the security of PHY and optimize secure communication. The impact of using AN and AI on an eavesdropper is evaluated using software-defined radio nodes.
%This study targets the entire physical link rather than a limited region and investigates the effectiveness of AN transmission gain at varying distances. Proper transmission gains are configured for AN transmission, and secure regions are established. The transmission of AI is considered on the receiver side, and AI analysis is crucial. The eavesdropper is implemented with two different devices: a robust device and a normal device with front-end drawbacks. The judicious use of AN yields secure regions, and real-time implementation showcases the model's applicability to real-life scenarios.

[S35] propose a novel physical layer authentication scheme for industrial wireless cyber-physical systems (CPS) using machine learning. This scheme, unlike traditional methods, doesn't rely on fixed thresholds. Instead, it utilizes channel matrices obtained from channel state information (CSI).

15/93 studies S8
[S6,S11
S14,
S20,
S25,
S34,
S35,
S50,
S51,
S52,
S53,
S57,
S58,
S92]


%\sha{Have we introduce this concept before? We have to define somewhere?} through a channel estimation process. The machine learning algorithm is then trained using both legitimate and illegitimate CSIs to accurately predict unauthentic channels.
%The approach represents a significant advancement in Physical Layer Authentication (PHY-AUC) for industrial wireless CPSs. It replaces conventional fixed threshold methods with Machine Learning (ML) algorithms, advocates for the use of channel matrices over channel differences, and suggests integrating Multiple-Input, Multiple-Output (MIMO) technology to enhance performance.
%Simulations and real-world validations confirm substantial performance improvements, particularly when employing the BT algorithm with 128-size matrices as inputs. Key findings include:
% (i) Implementation of MIMO technology greatly enhances performance, achieving near-perfect accuracy in specific positions and an average accuracy of 0.7710 across all positions.
% (ii) Authentication accuracy exhibits notable variation with position, decreasing as the distance between the legitimate transmitter and potential attacker increases.
% (iii) The BT-based Threshold-Free PHY-AUC (TF-PA) method, while offering superior accuracy, comes at the cost of significantly higher computational complexity and processing times. However, processing delays around 10 ms are deemed acceptable in certain scenarios.

%\paragraph{Human Sensing.}
%\sha{Why this is defensive strategies. Why this is useful? Start with that to get the attention. Maybe look at the intro of those papers and see a good use cases and mention here before going to details.}

%Traditionally, human detection with machine learning algorithms has been explored through the use of images and video data.
%Recent works suggest that radio frequency data are a viable alternative without the drawbacks of vision, such as occlusion, low-light conditions, and distance. 
%The work of \citep{khunteta2022rf} demonstrate the viability of using mmWave radar (22--77 Ghz) for human re-identification (HRI), human activity recognition (HAI) and surrounding location identification (SLI). 
%The authors employ a convolutional neural network (CNN) and Long Short-Term Memory (LSTM) network for HRI and SLI, and a hierarchical classifier for HAI. 
%The paper report high accuracy ($\geq 88\%$) for identifying 5 individuals, 5 rooms and 10 human activities within 1-6 meters of the mmWave radar. 

%\sha{These sounds like attack papers and maybe belong to eveasdroping attacks? DO we have good human sensing for authentication paper/s?} 
Another line of literature demonstrates that it is also possible to remotely eavesdrop on individuals using mmWave radar. A recent work by [S85] demonstrates that commercial off-the-shelf mmWave systems (TI AWR1843 BOOST (77 Ghz) and IWR6843ISK (60 Ghz)) can be used to remotely listen to phone calls using \textcolor{black}{ML}.
The system detects changes in phases of mmWave signals reflected from the body of the phone and is reportedly able to recognise digits and keywords.
The authors report an accuracy of 44-83\% in the range of 1-6 feet from the victim. 
In the work of \citep{wang2022mmeve}, the authors propose using a generative adversarial network (GAN) to extend the range of eavesdropping to 6-8 feet. 
The GAN reportedly removes environmental noise interfering with the original signal.
Another work demonstrates that by simply employing signal processing on mmWave radio, it is possible to reconstruct audio from moving sources at various distances including those with sound insulators [S20].
%\sha{We need to put here the IEEE SP'22, '23 here that I posted few weeks ago. David red those papers}
A more recent work by [S85] demonstrates that commercial off-the-shelf mmWave systems (TI AWR1843 BOOST (77 Ghz) and IWR6843ISK (60 Ghz)) can be used to remotely listen to phone calls using \textcolor{black}{ML}.
The system detects changes in phases of mmWave signals reflected from the body of the phone and is reportedly able to recognise digits and keywords.
The authors report an accuracy of 44-83\% in the range of 1-6 feet from the victim. 
In the work of \citep{wang2022mmeve}, the authors propose using a GAN to extend the range of eavesdropping to 6-8 feet. 
The GAN reportedly removes environmental noise interfering with the original signal.
Another work [S20] demonstrates that by simply employing signal processing on mmWave radio, it is possible to reconstruct audio from moving sources at various distances including those with sound insulators [S20].

These works suggest that there are significant privacy concerns with the introduction of higher frequency radio frequencies, as reportedly planned in the next generation of 6G. 
While these technologies are currently in their early stages, it is prudent to keep an eye on their development to ensure our preparedness.
%\sha{This seems good statement to end the eveasdropping attack subsection or something. We need fingerprinting or authentication for here. Sorry repeating to highlight the message? :)}




%\paragraph{ Eavesdropper Detection}

% \textcolor{black}{Please fill the references here, @Bushra, @David, @Nan }done by NW

% The detection of eavesdroppers in wireless networks has indeed been a longstanding and challenging issue in the field of cybersecurity. This problem stems from several factors:
% \begin{itemize}

    
%     \item \textbf{Inherent Challenges in Detecting Eavesdroppers}:  Detecting eavesdroppers in wireless networks is notably challenging because they can intercept communications without sending out any signals themselves. This means they can stay under the radar, often going undetected. They don't need to engage in obvious communication activities, making their presence hard to notice. This problem is highlighted in several research studies~\citep{chaman2018ghostbuster,atallah2019secrecy,din2018multiple}, which discuss how this stealthy nature of eavesdropping poses significant detection challenges.

%     \item \textbf{Technological Evolution Empowering Eavesdroppers}: As technology progresses, eavesdroppers get access to more advanced tools, which makes them even more efficient and harder to detect. They use state-of-the-art equipment and software to sneak into communications without being noticed. This evolution in eavesdropping capabilities, facilitated by technological advancements, is detailed in works like~\citep{li2021legitimate}.

%     \item \textbf{Vulnerabilities in Complex Wireless Networks}: Modern wireless networks are intricate and diverse, integrating a wide range of devices and communication methods. These include non-orthogonal multiple access (NOMA), full-duplex networks, massive multiple input multiple output (MIMO), cognitive radio networks, relay networks, simultaneous wireless information and power transfer (SWIPT), UAV communication networks, space information networks, and heterogeneous networks. Such complexity introduces numerous potential vulnerabilities that can be exploited by eavesdroppers.~\citep{alageli2023concurrent}.

%     \item \textbf{The Double-Edged Sword of Encryption}: While encryption is essential for protecting data, it also makes it difficult to tell the difference between legitimate users and eavesdroppers. When data is encrypted, both appear similar from the perspective of the network, making it challenging to identify malicious activity. This paradox of encryption is discussed in research like~\citep{trevisan2020does}.

%     \item \textbf{The Dynamic Nature of Wireless Signals}: The wireless environment is dynamic, with signals affected by various factors like distance, obstacles, and interference. This variability adds another layer of complexity to the detection of eavesdroppers~\citep{ye2022trust,al2020protecting,alsulami2021game}.

%     \item \textbf{Lack of Physical Boundaries}: Unlike wired networks, wireless networks are not confined by physical boundaries. This lack of physical limits makes it much easier for eavesdroppers to access the network from afar without needing to physically break into a system.

%     \item \textbf{Legal and Ethical Constraints}: Trying to detect eavesdroppers is not just a technical challenge but also involves legal and ethical considerations. There are strict privacy laws and regulations that limit how much network traffic can be monitored and analyzed for detecting eavesdroppers. This delicate balance between security and privacy is discussed in ~\citep{ning2020detection,timilsina2018secure}, highlighting the constraints faced in implementing monitoring strategies.
% \end{itemize}

% Given these challenges, the development of systems like EarFisher~\citep{262013}, which uses innovative techniques to detect eavesdroppers by analyzing memory EMRs, represents a significant advancement in this field. These systems are crucial for maintaining the security and integrity of wireless communications, especially in environments where sensitive information is transmitted. Continued research and development in this area are essential to keep pace with the evolving tactics of eavesdroppers and to safeguard against unauthorized access to wireless communications.

\subsubsection{Spoofing Attack}

Spoofing attacks represent a critical threat in spectrum management, involving the falsification of signals or data. These attacks are executed with the intent to deceive the spectrum management system. Spoofers often mimic legitimate users, which allows them to gain unauthorized access or misguide the system. Such actions can lead to incorrect spectrum allocation and pose risks to communication security.
In the domain of secure wireless communication, pilot spoofing attacks are particularly concerning, especially in scenarios involving beamforming. These attacks target the channel estimation processes, with the potential to severely disrupt them. The compromise of these processes can lead to significant security breaches in the physical layer of wireless transmissions, presenting a substantial challenge in maintaining secure communication.
To counter this threat, various innovative approaches have been developed:

[S4, S28,S6]


\begin{itemize}
\bushra{None of the mentioned references are in the data extraction form
    \item \textbf{Random Sequences and MDL Criterion}: A notable method involves the integration of random sequences in conjunction with the Minimum Description Length (MDL) criterion. This strategy is designed to enhance the detection of pilot spoofing attacks. The MDL criterion, a statistical model selection tool, helps in identifying the presence of spoofing by analyzing the characteristics of the received signal~\citep{chai2022ris,tugnait2018mitigation}.
    \item \textbf{Joint Estimation and Secure Beamforming}: Another effective technique encompasses the joint estimation of channels for both the legitimate receiver and potential eavesdroppers. This is coupled with secure beamforming strategies. Such an approach not only aids in identifying pilot spoofing attempts but also works towards mitigating their effects, thereby preserving the integrity of the transmission~\citep{tugnait2018pilot,tugnait2017detection}.
    \item \textbf{Utilization of Reconfigurable Intelligent Surfaces (RIS)}: The employment of RIS in training phases presents a forward-thinking solution. RIS can play a crucial role in detecting pilot spoofing attacks. Additionally, it enhances the achievable secrecy rates, an essential metric in assessing the effectiveness of secure communication systems. This is achieved by leveraging the ability of RIS to intelligently alter the propagation environment~\citep{tugnait2017mitigation}.}
    \item \textbf{Combating Spoofing Relay Attacks}:  Beyond pilot spoofing, the issue of spoofing relay attacks in beamforming also demands attention. Addressing this, techniques involving joint channel estimation and secure beamforming have been proposed. These methods not only detect but also effectively mitigate the impacts of such relay attacks, ensuring the secure transmission of data~\citep{tugnait2017mitigation2}. \bushra{Not included in the data extracted but fullfils the criteria}
\end{itemize}

These diverse strategies underline the evolving nature of secure communication technologies and the ongoing efforts to safeguard them against sophisticated threats like pilot spoofing and relay attacks. By continuously refining these techniques, the robustness of secure wireless communication systems against such vulnerabilities can be significantly enhanced.


% \textcolor{black}{Shuiqiao: we need some references here.} done by NW

% \begin{table}[h]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Strategy Type} & \textbf{Description} & \textbf{Reference} \\ \hline
% Robust AI Models & AI models resilient to attacks & [8] \\ \hline
% Fingerprinting Authentication & Using unique device characteristics for authentication & [9] \\ \hline
% Anomaly Detection & Identifying unusual patterns to detect threats & [10] \\ \hline
% \end{tabular}
% \caption{Defensive Strategies in Spectrum Management}
% \label{tab:defensive_strategies}
% \end{table}

\subsection{Defensive Strategies}
%These are  papers that talk about defence our SLR, these three can be added \citep{sharma2023secrecy,jere2023bayesian,dinh2023defensive}
[S5, S8, S11, S12, S20, S23, S24, S25, S27, S28, S31, S32, S33, S34, S35, S40, S45, S46, S47, S48, S49, S50, S51, S52, S53, S54, S56, S57, S58, S59, S60, S61, S92]

%\sha{We need some entry text here to prepare the reader for what's coming below!}

In this section, we focus on key defensive strategies for AISM, addressing various sophisticated threats. We'll start by examining robust AI models designed to resist adversarial attacks and data manipulations, essential for maintaining spectrum management integrity. Next, we delve into advanced fingerprinting methods for authentication, ensuring spectrum access is limited to verified users. We also cover privacy-preserving techniques vital for protecting sensitive data from direct attacks and unintended exposure. Additionally, we'll discuss anomaly detection methods acting as an early alert system to identify potential breaches. Lastly, we explore anti-jamming approaches using adaptive algorithms to maintain signal integrity against deliberate interference. 




% As the AI-enabled spectrum management landscape grapples with an array of sophisticated threats, from insidious AI attacks to pervasive physical layer assaults, the deployment of robust defensive strategies becomes paramount.
%  This critical section is dedicated to unpacking the arsenal of countermeasures designed to fortify the spectrum management ecosystem against these multifarious attacks.
 
%  In this section, we will introduce the relevant defensive strategies against different types of attacks.
%  We will explore the robust AI models, engineered to withstand adversarial attacks and data manipulations, are critical in ensuring the integrity of spectrum management.
%  Then, we explore the cutting-edge  fingerprinting for authentication emerges as a guardian of identity, ensuring that access to spectrum resources is restricted to verified users.
%  we will also examine privacy-preserving methods that are essential in safeguarding sensitive information from both direct attacks and collateral exposure. 
% Further,we explain anomaly detection techniques that serve as an early warning system, identifying deviations from normal patterns that could indicate a breach.
% Finally, we will explore anti-jamming tactics are also at the forefront, employing adaptive algorithms to preserve signal integrity amidst deliberate interference.

\subsubsection{Robust AI models}

%\subsection{Robust Channel Estimation Against Adversarial Attacks}

%The reliance on AI for spectrum management also exposes a new vulnerability; these models are susceptible to adversarial attacks. Sophisticated attackers can craft perturbations that, when introduced into the channel estimation input data, cause the AI models to make erroneous predictions.
%This fragility poses significant risks, potentially undermining the reliability and security of communication systems. 
%The ease with which these AI models can be misled is a pressing concern, driving the need for robust defensive mechanisms that ensure the integrity and trustworthiness of AISM.
%\sha{This seems an example focusing on channel estimation. Provide reference}

%\sha{Can we say a general comment about the robust AI models that been extensively studied in other fields like computer vision and natural language processing, but it is still in its infancy stage in the spectrum management space as AI also recently emerging in there? Use your own words :)}
%\sha{Why first paragraph is channel estimation? Lets try to be more general :)}
%\sha{This seems a bit more general paragraph. But this Robust AI models need to be restructured to start from general and give examples of few defensive strategies we identify} 
%In the quest to safeguard AI models in spectrum management against adversarial attacks, a plethora of defensive strategies have been developed and refined， such as adversarial training, input preprocessing, model regularization, etc.
%These strategies span from enhancing model robustness through adversarial training to leveraging the nuanced complexities of ensemble methods. Each approach offers a unique line of defense, aiming to shield AI systems from the cunning manipulations posed by adversaries. Amidst these varied tactics, one particular strategy that stands out for its effectiveness and ingenuity is the use of model distillation for defensing agaist adversarial attacks in Spectrum management. 

%\sha{This looks like good paragraph to start with. Profide references.}

The current landscape of spectrum management reveals a concerning vulnerability in AI models. Unlike in computer vision, where defensive strategies against adversarial attacks have seen extensive development and implementation, the approaches in spectrum management are comparatively nascent and limited. This discrepancy highlights a significant gap in the field: while AI models in computer vision are increasingly fortified against attacks through techniques like adversarial training, network distillation, and robust feature extraction, similar comprehensive defensive frameworks are conspicuously lacking in spectrum management. Currently, there are few works working on robust AI models for spectrum management. Table \ref{tab:defense_strategies_attacks} summarizes key references for the robust AI models. 

\begin{table}[h]
\centering
\begin{tabular}{|l|p{6cm}|l|}
\hline
\textbf{Type of Attack} & \textbf{Defense Strategies} & \textbf{Key References} \\ \hline
Adversarial Example Attacks & Defensive distillation to train robust AI models, especially in 5G wireless communications. & [S56] \\ \hline
Evasion Attacks & Subset feature selection with ensemble-based learning, and the Underlying Server Defense of Federated Learning (USD-FL). & \citep{wang2023mitigating} \\ \hline
Data Poisoning Attacks & Introducing incorrect transmissions, leveraging online quality learning, and using median/max influence estimation-based data aggregation. & [S32]\citep{ zhao2021data} \\ \hline
Backdoor Attacks & Anomaly detection algorithms, robust statistical methods, and integrating ML algorithms with network operation systems. & \citep{khaddaj2023rethinking, kolouri2020universal, hayase2021spectre, xia2022enhancing} \\ \hline
\end{tabular}
\caption{Defense Strategies for Different Types of Attacks in Spectrum Management}
\label{tab:defense_strategies_attacks}
\end{table}


\paragraph{Defense Strategies against Adversarial Example Attacks}

CATAK et al. [S56] presents an in-depth analysis of defensive distillation as a method for improving the robustness of deep learning models against adversarial attacks. 
Defensive distillation, a concept that originates from the field of knowledge distillation, involves training a complex teacher network and then transferring its knowledge to a simpler student network by softening the softmax output probabilities with a temperature parameter. This technique has been shown to make the resulting models less susceptible to adversarial examples, which are inputs designed to fool the model into making incorrect predictions. The paper details the implementation of this methodology within the realm of 5G wireless communications, particularly for the task of channel estimation. By leveraging MATLAB's 5G Toolbox, the researchers synthesize a diverse dataset representing various channel conditions to train a convolutional neural network (CNN). This allows for the creation of a student model capable of estimating wireless channels with improved defense against adversarial attacks, ensuring more reliable communication.

\paragraph{Defense Strategies against Evasion Attacks}

In the realm of IIoT, the battle against sophisticated evasion attacks has led to the development of several innovative defense strategies. A prominent approach is the utilization of subset feature selection combined with ensemble-based learning. This technique is specifically engineered to identify and neutralize fabricated attacks, thereby bolstering the resilience of systems against advanced malware~\citep{wang2023mitigating}. Another significant advancement is the Underlying Server Defense of Federated Learning (USD-FL). This specialized framework is designed to protect FL-based signal classifiers, offering enhanced defense capabilities against model poisoning threats inherent in FL systems~\citep{wang2023mitigating}.
Furthermore, the growing dependency on AI-based semantic segmentation models for spectrum sensing in cellular networks has revealed new vulnerabilities. Recent studies analyzing these vulnerabilities have highlighted an urgent need for effective mitigation strategies. These strategies are essential in minimizing the systems' vulnerability to adversarial attacks, which could otherwise exploit these weaknesses, potentially leading to disruptions in network operations [S24]



\paragraph{Defense Strategies of Data Poisoning Attacks}

% A novel dynamic defense mechanism has been developed to counter Data poisoning attacks on transmitters. This strategy involves the transmitter deliberately making a limited number of erroneous transmissions. The intention behind these 'mistakes' is to disrupt the adversary's training data, thereby deceiving them and undermining their attack strategy. This method not only confuses the adversary but also ensures that the transmitter maintains its throughput levels, effectively securing spectrum management against data poisoning for more reliable communication.

To defend against data poisoning attacks in spectrum management, dynamic and intelligent strategies are essential. One effective tactic is the intentional introduction of incorrect transmissions by the targeted transmitter, aimed at distorting the adversary's training data to render their attack ineffective. The primary objective of this strategy is to maintain the transmitter's throughput, thus ensuring uninterrupted and reliable communication [S32] 

Additionally, another defense mechanism involves leveraging online quality learning, especially useful in crowdsourcing contexts. This approach focuses on identifying and neutralizing the influence of malicious contributors offering low-quality or deceptive data. By distinguishing and mitigating these unreliable sources, the integrity of the data aggregation process is preserved [S32].

\bushra{[Not related to spectrum management adversarial defense] Further augmenting these strategies is the implementation of median and maximum influence estimation-based data aggregation. This technique aggregates data in a manner that minimizes the impact of outliers and potentially poisoned inputs. Concentrating on median or maximum influence estimations allows for a more accurate discernment of genuine data trends, significantly reducing the effects of data poisoning attacks~\citep{zhao2021data}.} 

\bushra{[Not meeting inclusion and exclusion criteria]
These varied defense mechanisms have proven effective in reducing the adverse effects of data poisoning attacks and in maintaining the accuracy and reliability of critical data in spectrum management. Representing a proactive and comprehensive approach to cybersecurity, these strategies are tailored to meet the unique challenges of spectrum data manipulation~\citep{shi2018spectrum}.}

\paragraph{Defense Strategies of Backdoor Attacks}

%Backdoor attacks present a serious threat to the security and integrity of wireless networks, leading to risks like unauthorized access, data breaches, misinformation, and service disruptions. To counter these challenges, innovative solutions are being developed. Advanced detection methods, including anomaly detection algorithms, are employed to spot unusual patterns indicative of backdoor attacks. \textcolor{black}{ML} models are also being trained to recognize and counter these threats, thus enhancing network resilience.

%A practical strategy is to treat malicious examples in the training set as outliers. 
Robust statistical methods are applied to identify and remove these outliers, purifying the training dataset from malicious influences~\citep{khaddaj2023rethinking}. Another approach assumes that backdoor attacks are linked to the most significant features in the training data. Developing an algorithm that identifies these dominant features can help uncover and mitigate backdoor attacks~\citep{kolouri2020universal}.

Robust covariance estimation is another technique used to accentuate the spectral signature of corrupted data. This strategy aids in differentiating genuine data from tainted data, facilitating the creation of a model free from backdoor influences~\citep{hayase2021spectre}. 
%The method of difference reduction has also been proposed. This involves integrating multi-level Maximum Mean Discrepancy (MMD) regularization into the loss function to diminish distributional differences between benign and malicious samples, thus improving the effectiveness of difference-based defense strategies~\citep{xia2022enhancing}.

%Looking to the future, advancements could involve integrating \textcolor{black}{ML} algorithms with network operation systems for ongoing threat monitoring and adaptation. The development of automated systems capable of learning from detected threats and updating defense mechanisms in real-time would greatly enhance network resilience. Furthermore, incorporating these detection methods into broader cybersecurity frameworks could offer a more comprehensive defense, ensuring robust protection against various cyber threats in wireless communication networks.


% \paragraph{Defense Strategies of Backdoor Attacks}

% These various forms of backdoor attacks pose a grave threat to the security and integrity of wireless networks. They can lead to unauthorized access, data breaches, misinformation, and disruption of network services. In response to these challenges, novel solutions are being developed and implemented. Advanced detection methods, like anomaly detection algorithms, can be used to identify unusual patterns that may be indicative of a backdoor attack. Machine learning models are also being trained to recognize and neutralize these triggers, enhancing the network's resilience against such threats.
% One effective approach involves treating the malicious examples inserted into the training set as outliers. Robust statistical techniques can be applied to identify and eliminate these outliers, thereby cleansing the training dataset of any malicious influences~\citep{khaddaj2023rethinking}.
% A different approach is based on the assumption that backdoor attacks correspond to the most prominent features in the training data. By developing a detection algorithm that focuses on identifying these dominant features, it's possible to uncover and mitigate the effects of backdoor attacks~\citep{kolouri2020universal}.
% Additionally, robust covariance estimation can be utilized to amplify the spectral signature of corrupted data. This method enhances the differentiation between genuine and tainted data, facilitating the development of a clean model that is free from backdoor influences~\citep{hayase2021spectre}.
% A method involving difference reduction has been proposed, which incorporates multi-level Maximum Mean Discrepancy (MMD) regularization into the loss function. This approach aims to reduce the distributional differences between benign and malicious samples, thereby improving the efficacy of difference-based defense methods. This method adds another layer of sophistication to backdoor attack detection, enhancing the overall security of the system~\citep{xia2022enhancing}.
% Extending these methods, future advancements could focus on the integration of machine learning algorithms with network operation systems to continuously monitor and adapt to new threats. The development of automated systems that can learn from detected threats and update defense mechanisms in real-time would significantly enhance network resilience. Moreover, incorporating these detection methods into larger cybersecurity frameworks could provide a more holistic defense strategy, ensuring robust protection against a range of cyber threats in wireless communication networks.


\subsubsection{Fingerprinting Authentication}
%\sha{We need to pitch as saying while mmwave could be used for eveasdroping, it also has useful use which is authenticating humans and devices very accurately?} 

%As we navigate the complex terrain of securing devices within the realm of spectrum management, the traditional reliance on cryptographic methods, while essential, is increasingly complemented by more nuanced and sophisticated techniques. Among these, 
Radio frequency fingerprinting, also known as specific emitter identification (SEI), emerges as a pioneering approach. This technique capitalizes on the unique characteristics inherent in radio signals emitted by wireless devices, akin to a digital fingerprint. Each device, due to its distinct hardware and transmission properties, leaves an indelible mark on the signals it emits—a mark as unique as a human fingerprint.

%The development of advanced mobile communication networks and machine learning algorithms has enabled a potentially transformative technology: the ability to detect the presence of humans and devices using raw radio frequency signals.
%Like the Radio Detection and Ranging (RADAR) system that was introduced in 1930s for navigation and defense, the modern application of radio frequency sensing within 6G mobile networks has the potential to revolutionize smart cities, urban planning and physical security, however raises many privacy concerns. 
Recently many authors report successfully applying \textcolor{black}{ML} algorithms over several radio frequency modalities (e,g, mmWave, WiFi, RFID and ZigBee) to solve problems with privacy concerns, such as human re-identification [S1] or remote eavesdropping [S20]. 
In comparison to traditional sensing technologies, such as optical cameras, radio frequency signals can penetrate walls and are unaffected by weather and lighting conditions. 
%A common observation amongst many authors is that higher frequencies result in improved machine learning performance.In particular, the rapid development of millimeter wave (mmWave) sensors has attracted much attention, leading to the emergence of mmWave sensing technology. These signals operate at a higher frequency (30-300Ghz) and have a larger bandwidth which provides higher sensing sensitivity and precision. The greater resolution and bandwidth allows machine learning algorithms to better distinguish between objects in the data. Furthermore, shorter wavelengths allow for smaller antenna which can be tightly integrated into smaller physical spaces. Newer technologies, such as beamforming or Multiple Input Multiple Output (MIMO), also enhance the directionality and transmission gain. The next generation of 6G mobile networks are anticipated to harness the potential of terahertz (THz) frequencies which will likely improve machine learning performance of use-cases proposed in existing literature. Below, we provide an overview of existing literature encompassing human and device sensing with radio frequencies.  
%\paragraph{Device Sensing.}
%\sha{The pitch here seems better subsection than the previous.}
%Cryptography methods are currently the predominant form of detecting and authenticating devices within a modern computer network. 
%These methods, while highly secure and resistant to various attacks, often demand processing power that surpasses what many Internet-of-Things (IoT) devices. 
%As we edge closer to the advent of 6G networks, the limitations in computational resources of IoT devices could potentially create exploitable vulnerabilities.  
%Moreover, the reliance on cryptographic methods carries an inherent risk of spoofing attacks, particularly if encryption keys fall into the attacker's hands.

%An emerging technique to complement cryptography methods and address these concerns is \textbf{radio frequency fingerprinting}, also known as\textbf{ specific emitter identification} (SEI).
%These family of techniques employ a \textcolor{black}{ML} algorithm to learn the  unique radio frequency signature emitted by a specific device.
%Each device contains unique hardware imperfections imparted during the manufacturing process, such as the minor variations in oscillator frequencies, slight deviations in transistor characteristics, or small differences in printed circuit board traces, which can all contribute to a distinctive RF signature. 
%This signature, often termed a device's "fingerprint," can be detected and used to identify individual devices among many, even if they are of the same make and model.
The largest study of RF fingerprinting to date by \citep{jian2020deep} shows that open-source convolutional neural networks can identify up to 100 devices using their WiFi signals at an accuracy of 83.5\%. 
The experiment results reveal that accuracy drops if the number of devices increases (up to 10k devices shown) or if the number of transmissions per device within the training dataset decreases. 
Another work [S4] demonstrates that RF fingerprinting can mitigate the risk of base station spoofing attacks on industrial IoT devices. 
The authors show that a conventional convolutional neural network can identify signals from 3 base stations with up to 99\% accuracy in a real-world dataset collected from a university campus. 

% \begin{table}[h]
% \centering
% \begin{tabular}{|l|p{6cm}|l|}
% \hline
% \textbf{Aspect} & \textbf{Details} & \textbf{Key References} \\ \hline
% Traditional Methods & Traditional spectrum management like database-driven dynamic spectrum sharing faces flexibility and vulnerability issues. & \citep{li2019comparison} \\ \hline
% Challenges with Traditional Methods & Differential privacy techniques in social network graph construction lack complete privacy protection. & \citep{liu2021spectrum} \\ \hline
% Resource-Efficient Privacy Solution & Development of a lightweight solution for spectrum aggregation and auctions, focusing on user location privacy. & \citep{zhou2019ppsas} \\ \hline
% Blockchain-Based Framework & A blockchain framework for dynamic spectrum access systems, offering decentralization, transparency, and immutability. & \citep{tu2020blockchain} \\ \hline
% Trust-Based System & A trust-based system for spectrum allocation with a Proof-of-Trust consensus mechanism. & \citep{ye2022trust} \\ \hline
% Techniques for Sensitive Users & Methods like obfuscation and trust-based location protection for secure spectrum access. & \citep{wang2020efficient} \\ \hline
% \end{tabular}
% \caption{Privacy-Preserving Methods in Spectrum Management}
% \label{tab:privacy_preserving_methods}
% \end{table}


\subsubsection{Privacy-Preserving Method in Spectrum Management}

This subsection explores the vital role of privacy-preserving methods in AISM, particularly pertinent in IoT networks. In an era reliant on extensive datasets, safeguarding privacy goes beyond regulatory compliance; it's crucial for maintaining user trust and security. These methods, from blockchain technology to cryptographic techniques, aim to protect sensitive data in environments characterized by significant data sharing and collaborative decision-making.

\textbf{Traditional Methods and Their Challenges:} Traditional spectrum management methods, like database-driven dynamic spectrum sharing, encounter flexibility and vulnerability issues~\citep{li2019comparison}. The employment of differential privacy techniques in social network graph construction, while innovative, falls short in ensuring complete privacy protection~\citep{liu2021spectrum}.

\textbf{Recent Developments in Privacy-Preserving Techniques:}
\begin{itemize}
    \item \textbf{Resource-Efficient Privacy Solution:} A focus on resource efficiency led to the development of a lightweight solution for spectrum aggregation and auctions, prioritizing user location privacy—ideal for resource-constrained networks~\citep{zhou2019ppsas}.
    % \item \textbf{Yanjiao et al.'s Cryptographic Techniques:} Delving into cryptographic methods for spectrum auction design, this approach aims to safeguard participant information while maintaining a fair and functional auction process~\citep{chen2019privacy}.
    \item \textbf{Blockchain-Based Framework:} In addressing dynamic spectrum sharing challenges, a blockchain-based framework was introduced, leveraging its decentralization, transparency, and immutability for dynamic spectrum access systems~\citep{tu2020blockchain}. Further, Ye et al. revolutionized spectrum allocation with a trust-based system, integrating a Proof-of-Trust consensus mechanism for enhanced security and reliability in DSA~\citep{ye2022trust}.
    \item \textbf{Techniques for Sensitive Government Incumbent Users:} To address heightened privacy concerns, methods like obfuscation and trust-based location protection were proposed, ensuring efficient yet secure spectrum access~\citep{wang2020efficient}.
\end{itemize}

These innovative approaches symbolize a convergence of privacy, efficiency, and functionality—key elements for the upcoming 6G era. They address current challenges in spectrum management and lay the groundwork for advanced, secure, and efficient spectrum resource management in the future 6G landscape. This amalgamation of cutting-edge research with 6G technology is a proactive step towards robust, secure, and optimized wireless communication for the future.



\subsubsection{Anomaly Detection in Spectrum Management}

Spectrum management, a complex task of allocating frequency bands for reliable communication, faces the challenge of detecting and mitigating anomalies. These anomalies can range from unauthorized access and interference to signal degradation, equipment malfunctions, and malicious attacks.
Anomaly detection is vital for maintaining the integrity, security, and performance of 5G and beyond networks. It leverages AI and ML to monitor and analyze the spectrum environment, identifying deviations from expected behavior, thus enabling swift responses to threats or issues and ensuring seamless connectivity.

\textbf{Innovative Approaches in Anomaly Detection:}
\begin{itemize}
    \item \textbf{Two-Tiered Deep Learning Architecture (Maim{\'o} et al.):} A novel approach using a two-tiered deep learning architecture for anomaly detection in 5G networks is presented~[S59]. The first tier, the Anomaly Symptom Detection (ASD) module, classifies network traffic as normal or potentially anomalous. The second tier, the Network Anomaly Detection (NAD) module, employs an LSTM network for a detailed classification of the traffic.
    \item \textbf{Optimized Structure for 6G Networks (Han et al.):} A method optimized for 6G networks introduces a three-layer structure for IIoT, enhancing data reliability and early detection of critical events [S54]. This system uses advanced anomaly detection methodologies, like ARX models and OCSVM, to filter out noise and prioritize data relevance, crucial for URLLC in 6G networks.
    \item \textbf{Credibility Assessment and Time-Series Analysis (Zhang et al.):} A Bayesian reputation model for urban sensor networks that improves anomaly detection by evaluating sensor nodes' credibility and incorporating a time forgetting factor and aggregate credibility measure~[S60]. This method is vital for maintaining the integrity of urban sensing data in smart cities.
    \item \textbf{Fault-Tolerant Event Region Detection (Li et al.):} An advanced algorithm using Gaussian Mixture Models (GMMs) for fault-tolerant event region detection in WSNs [S61]. This approach differentiates between environmental phenomena and sensor faults, supporting autonomous decision-making in 6G.
\end{itemize}

% The continuous evolution of wireless networks, particularly with the advent of 6G, necessitates robust anomaly detection mechanisms. These innovations not only address current spectrum management challenges but also set the foundation for efficient, secure, and reliable network operations in the future of wireless communication.


% \subsubsection{Anomaly Detection}

% Spectrum management is a complex task that involves allocating and coordinating frequency bands to ensure reliable and interference-free communication for a multitude of devices and services. In this dynamic and highly congested spectrum landscape, the ability to detect and mitigate anomalies is paramount. Anomalies can encompass a wide range of issues, including unauthorized access, interference, signal degradation, equipment malfunctions, and even malicious attacks on the network.
% Anomaly detection plays a pivotal role in maintaining the integrity, security, and performance of 5G and beyond networks. It leverages the power of artificial intelligence (AI) and machine learning (ML) to continuously monitor and analyze the spectrum environment, identifying deviations from expected behavior. By doing so, anomaly detection systems enable swift responses to emerging threats or issues, ensuring seamless and uninterrupted connectivity for users and applications.
% This introduction sets the stage for a closer exploration of anomaly detection in 5G and beyond for spectrum management. We will delve into the various challenges, emerging technologies, and real-world applications that make anomaly detection a critical component of spectrum management in the era of next-generation wireless networks.


%\paragraph{Anomaly Detection for Spectrum Management}
%\sha{This part seems relvent but a bit generic. We need to say what existing anomaly detection methods are specifically looking at. WHat's the legit behavior in the spectrum management? What the advesrasy trying to do? What they target? Are they targeting individuals? base stations or other 5G components? That's important to explain up front and then connect the below papers to that.}

%Anomaly detection systems are crucial for identifying potential security breaches and threats within a network. Efficiently managing and protecting the spectrum requires robust network security measures to prevent malicious activities that can disrupt service, such as unauthorized access or denial of service attacks, which can also include illegal use of the spectrum.

% Maim{\'o} et al.  [S59] presents a two-tiered deep learning architecture for anomaly detection within 5G networks, aimed at balancing the high-speed requirements of 5G data processing with the need for accurate identification of security threats. The first level of this system is the Anomaly Symptom Detection (ASD) module, which quickly classifies network traffic flows as normal or potentially anomalous, using feature vectors calculated from the traffic data. Speed is paramount at this level, even at the expense of some accuracy.
% The potentially anomalous flows are passed to the second level, the Network Anomaly Detection (NAD) module, which employs an LSTM network to conduct a more thorough analysis of the symptom sequences. The NAD is responsible for the detailed classification of the traffic into various categories of attacks or anomalies.
% In essence, the proposed system showcases the application of deep learning to address the dual challenges of speed and accuracy in the anomaly detection process within the rapidly evolving domain of 5G networks. The architecture leverages the strengths of different deep learning models to process vast amounts of network data swiftly, while also ensuring that detailed, accurate detection is not compromised in the subsequent, more in-depth analysis stage.
% The detection of anomalies could lead to insights and actions that are beneficial for the optimal allocation and use of spectrum resources.

% The paper [S54] presents a method tailored for sixth-generation (6G) networks. The paper introduces an optimized three-layer structure for the Industrial Internet of Things (IIoT), specifically refined to leverage the capabilities of upcoming 6G technology. At its core, the model aims to streamline the data flow from IIoT nodes through an SDN-managed perception layer, via a 6G-enabled network layer, and ultimately to the application layer for processing and analysis on cloud servers. Enhanced by a novel anomaly detection methodology that exploits spatiotemporal correlations, the system distinguishes between valuable data and outliers using a sophisticated Autoregressive with eXogenous inputs (ARX) model in tandem with a One-Class Support Vector Machine (OCSVM). This approach not only improves data reliability by filtering out noise and errors but also aids in the early identification of system-critical events, ensuring the integrity and utility of the data harvested from the IIoT landscape.
% Within the ambit of spectrum management, this enhanced IIoT framework is a harbinger of the efficiency and reliability that 6G networks aim to deliver. By employing edge computing and intelligent data filtering, the model anticipates the vast data influx characteristic of 6G, enabling more judicious use of the spectrum while meeting stringent low-latency and reliability requirements. The system's ability to discern and prioritize information relevance effectively maximizes spectrum utility, a cornerstone in the realization of 6G's promise for ultra-reliable low-latency communications (URLLC). Consequently, the proposed model not only elevates the operational proficiency of IIoT networks but also serves as a crucial blueprint for managing the precious spectral resources in the hyper-connected era of 6G.


% Zhang et al. [S60] proposes a novel anomaly detection framework for urban sensor networks, enhancing reliability by integrating credibility assessment and time-series analysis. The paper addresses the challenge of detecting anomalies in data collected by urban sensor networks, where sensors can generate abnormal data due to various reasons, such as equipment failure, external attacks, or special environmental event.
% To address the limitations of traditional threshold-based approaches, they develop a Bayesian reputation model that evaluates sensor nodes' credibility based on historical data variance and mean, refining detection accuracy through dynamic Beta distribution updating. The method also includes a time forgetting factor to weigh recent data more heavily, and an aggregate credibility measure from neighboring nodes to set anomaly thresholds. This comprehensive model aims to improve the rate of true anomaly detection while minimizing false positives, promising better performance in maintaining the integrity of urban sensing data crucial for smart city applications.
% With 6G's expected improvements in edge computing and Internet of Things (IoT) integration, urban sensors will generate massive data streams in real-time, necessitating robust anomaly detection algorithms to maintain system integrity and performance. The paper's methodology could help ensure that 6G networks remain reliable and trustworthy by quickly identifying and responding to data anomalies, thereby supporting the efficient operation of smart cities. These capabilities are crucial for the health of 6G networks, where anomalies could signify network failures, security breaches, or other critical issues that need immediate attention.

% 6G networks will likely rely heavily on ultra-dense WSNs for a variety of applications, including environmental monitoring, smart cities, and IoT deployments. The massive scale and the complexity of the data generated by such networks demand robust and intelligent fault detection mechanisms to ensure reliability and accuracy.
% The ability to accurately identify the state of a sensor and distinguish between a faulty sensor and an environmental event is critical for the autonomous decision-making capabilities required in 6G. Furthermore, the low-latency and high-reliability communication promised by 6G will enhance the performance of such fault-tolerant detection algorithms, allowing for near-real-time diagnostics and response, which is essential for time-critical applications.
% Li et al. \citep{liu2019fault}  describes an advanced algorithm for fault-tolerant event region detection in Wireless Sensor Networks (WSNs). They introduce a method that utilizes Gaussian Mixture Models (GMMs) to understand and categorize the changes in sensor readings due to environmental changes or sensor faults. This is particularly useful in distinguishing between legitimate environmental phenomena and various types of sensor faults, such as persistent and transient 'suck-at' errors, where a sensor may be stuck at a high ('one') or low ('zero') reading.

% Building upon the foundation laid by anomaly detection techniques, the next critical aspect of securing wireless networks is the detection of eavesdroppers. Eavesdropper detection is paramount in safeguarding confidential communications from unauthorized interception. This is especially crucial in the era of 5G and 6G networks, where the exponential increase in connected devices and the complexity of communication protocols significantly elevate the risk of eavesdropping. The following section will delve into the various strategies and technological advancements being deployed to detect and mitigate the risks posed by eavesdroppers, thereby fortifying the security framework essential for modern wireless networks.

%The relentless evolution of wireless networks, particularly with the emergence of 6G technology, necessitates advanced anomaly detection systems. These systems are integral to addressing the challenges in current spectrum management and setting a foundation for future network operations that are efficient, secure, and reliable. A crucial extension of this security framework is eavesdropper detection, which is paramount in safeguarding confidential communications against unauthorized interception. This aspect gains even more significance in the 5G and 6G era, marked by a dramatic increase in connected devices and complex communication protocols, thereby elevating the risks associated with eavesdropping. The upcoming section will delve into the array of strategies and technological advancements aimed at detecting and mitigating the threats posed by eavesdroppers, further solidifying the essential security infrastructure of modern wireless networks.

% \begin{table}[h]
% \centering
% \begin{tabular}{|l|p{6cm}|l|}
% \hline
% \textbf{Challenge} & \textbf{Description} & \textbf{Key References} \\ \hline
% Inherent Challenges & Detecting eavesdroppers is difficult due to their silent, signal-less interception of communications. & \citep{chaman2018ghostbuster, atallah2019secrecy, din2018multiple} \\ \hline
% Technological Evolution & Eavesdroppers use advanced tools for stealthy communication interception, becoming more efficient and harder to detect. & \citep{li2021legitimate} \\ \hline
% Network Vulnerabilities & Complex wireless networks with diverse technologies create multiple vulnerabilities that eavesdroppers can exploit. & \citep{alageli2023concurrent} \\ \hline
% Encryption Paradox & Encryption, while protecting data, makes it hard to differentiate between legitimate users and eavesdroppers. & \citep{trevisan2020does} \\ \hline
% Dynamic Wireless Signals & The variability of wireless signals adds complexity to detecting eavesdroppers. & \citep{ye2022trust, al2020protecting, alsulami2021game} \\ \hline
% Lack of Physical Boundaries & Wireless networks' lack of physical limits allows easier access for eavesdroppers. & - \\ \hline
% Legal and Ethical Constraints & Legal and ethical limitations restrict the extent of network traffic monitoring for eavesdropper detection. & \citep{ning2020detection, timilsina2018secure} \\ \hline
% \end{tabular}
% \caption{Challenges in Eavesdroppers Detection in Wireless Networks}
% \label{tab:eavesdroppers_detection}
% \end{table}

\paragraph{Eavesdroppers Detection}
The detection of eavesdroppers in wireless networks has indeed been a longstanding and challenging issue in the field of cybersecurity. This problem stems from several factors:
\begin{itemize}

    \item \textbf{Inherent Challenges in Detecting Eavesdroppers}:  Detecting eavesdroppers in wireless networks is difficult because they can intercept communications silently, often remaining undetected. Unlike active communicators, they don't emit signals, making their presence hard to spot. This stealthy nature of eavesdropping, as discussed in various research studies~\citep{chaman2018ghostbuster,atallah2019secrecy,din2018multiple}, presents significant detection challenges.

    \item \textbf{Technological Evolution Empowering Eavesdroppers}: Advancements in technology have made eavesdroppers more efficient and harder to detect, as they now use sophisticated tools and software to stealthily intercept communications. This evolution in eavesdropping techniques, driven by technological progress, is outlined in studies like~\citep{li2021legitimate}.

    \item \textbf{Vulnerabilities in Complex Wireless Networks}: Modern wireless networks, with their complexity and diversity, incorporate various devices and communication techniques. These range from non-orthogonal multiple access (NOMA) and full-duplex networks to massive MIMO, cognitive radio networks, relay networks, and more, including SWIPT, UAV communication networks, space information networks, and heterogeneous networks. This complexity creates many vulnerabilities that eavesdroppers could exploit~\citep{alageli2023concurrent}.

    \item \textbf{The Double-Edged Sword of Encryption}: While encryption is essential for protecting data, it also makes it difficult to tell the difference between legitimate users and eavesdroppers. When data is encrypted, both appear similar from the perspective of the network, making it challenging to identify malicious activity. This paradox of encryption is discussed in research like~\citep{trevisan2020does}.

    \item \textbf{The Dynamic Nature of Wireless Signals}: The wireless environment is dynamic, with signals affected by various factors like distance, obstacles, and interference. This variability adds another layer of complexity to the detection of eavesdroppers~\citep{ye2022trust,al2020protecting,alsulami2021game}.

    \item \textbf{Lack of Physical Boundaries}: Unlike wired networks, wireless networks are not confined by physical boundaries. This lack of physical limits makes it much easier for eavesdroppers to access the network from afar without needing to physically break into a system.

    \item \textbf{Legal and Ethical Constraints}: Trying to detect eavesdroppers is not just a technical challenge but also involves legal and ethical considerations. There are strict privacy laws and regulations that limit how much network traffic can be monitored and analyzed for detecting eavesdroppers. This delicate balance between security and privacy is discussed in ~\citep{ning2020detection,timilsina2018secure}, highlighting the constraints faced in implementing monitoring strategies.
\end{itemize}

%Given these challenges, the development of systems like EarFisher~\citep{shen2021earfisher}, which uses innovative techniques to detect eavesdroppers by analyzing memory EMRs, represents a significant advancement in this field. These systems are crucial for maintaining the security and integrity of wireless communications, especially in environments where sensitive information is transmitted. Continued research and development in this area are essential to keep pace with the evolving tactics of eavesdroppers and to safeguard against unauthorized access to wireless communications.


\subsubsection{Anti-Jamming}


In the multifaceted domain of spectrum management, the threat of jamming presents a formidable challenge, necessitating the development and deployment of effective anti-jamming strategies. %Jamming attacks, characterized by the deliberate transmission of interfering signals, are designed to disrupt or deny the legitimate use of the spectrum, thereby compromising the integrity and reliability of communication systems. The importance of anti-jamming measures in this context cannot be overstated, as they are crucial for ensuring uninterrupted and secure wireless communication, especially in critical applications spanning from commercial networks to military communications.
%In the ever-evolving field of spectrum management, addressing the threat of jamming attacks stands as a crucial task to ensure reliable and secure communications. This section explores the forefront of anti-jamming strategies, particularly focusing on the integration of advanced technologies like AI, \textcolor{black}{ML}, and sophisticated algorithmic approaches to counter these threats effectively.

One innovative approach in this realm is the use of frequency hopping combined with reinforcement learning, an intelligent strategy that dynamically adapts to changing conditions and jamming patterns. This technique allows communication systems to continually shift frequencies, making it difficult for jammers to disrupt the signal persistently. The use of reinforcement learning in this context enables the system to learn from its environment and make informed decisions about frequency changes, enhancing its resistance to jamming over time.
Liu et al. \citep{liu2019pattern} have taken this concept further by proposing a sequential deep reinforcement learning algorithm (SDRLA) for anti-jamming communication. Their approach, which combines deep learning and reinforcement learning, is tailored to recognize and respond to specific jamming patterns. This results in a system that is not only reactive but also predictive in its anti-jamming measures, capable of operating effectively in dynamic and intelligent jamming environments. The use of SDRLA, particularly in the context of a 20MHz frequency band with specific frame lengths and transmission times, demonstrates improved performance and convergence compared to traditional single-mode reinforcement learning approaches.

Another significant contribution to the field comes from Van et al. \citep{van2019jam}, who focus on enhancing the deep Q-learning algorithm with a replay memory mechanism. This technique allows the system to learn efficiently from past experiences by removing correlations between observations, thereby stabilizing the learning process. Additionally, the incorporation of a target Q-network aids in stabilizing the value estimations during the training process, providing a more consistent and reliable learning environment for the AI model.

Van et al. \citep{van2021deepfake} have also introduced an intriguing concept termed 'DeepFake', a deep reinforcement learning-based deception strategy designed to counteract reactive jamming attacks. By generating fake signals to mislead jammers and simultaneously using these jamming signals to bolster system performance, this strategy offers a dual advantage. The deep dueling neural network architecture employed in DeepFake enables the system to learn an optimal policy for defeating reactive jamming attacks, as demonstrated through extensive simulations.
These studies collectively illustrate the potential of AI and \textcolor{black}{ML} in revolutionizing anti-jamming strategies in spectrum management. By leveraging these advanced technologies, spectrum management systems can enhance their resilience against jamming, ensuring uninterrupted and secure communications across various domains.    

%\sha{The subsection title is anti-Jamming but the first sentence below talking about eveasdropping?? These are two different islands. Also the listed items seems like too generic. Please rewrite. Thanks}



% NAN 





    




%bushra added backup
% \textbf{Model Hardening} is the most frequent defense applied to handle adversarial attacks. It has been used in seven studies across all types of adversarial attacks identified in this SLR. For instance, the defense strategy discussed in [S18] focuses on enhancing the robustness of FIRE against adversarial attacks, specifically those utilizing Universal Adversarial Perturbations (UAP). This is achieved through \emph{adversarial training} that incorporates batch-wise perturbations generated by the RW-PGD algorithm, selected for its strength and relevance in defending against UAP-based attacks. During training, each batch undergoes five random attacks with a 10\% budget, applied before the learning process. This defense method, despite extending training time, notably enhances the model's resilience against RAFA attacks, as evidenced by a robust model maintaining a higher average channel SNR even under a 30\% attack budget. This suggests adversarial training as a promising approach for creating more secure systems.
% Similarly, [S33 presents a defense that enhances the resilience of wireless signal classification against adversarial perturbations through the use of \emph{randomized smoothing}. This technique augments the training dataset with Gaussian noise, adjusting the model to be robust to such perturbations seen during testing. The defense strategically manipulates two parameters: the Gaussian noise's standard deviation and the count of noise-augmented samples, aiming to strike a balance between accuracy and robustness. Furthermore, it employs a certified defense for testing, utilizing statistical tests to confirm the classifications' reliability under adversarial conditions. This approach not only counters the effects of adversarial attacks but can also improve the classifier's performance by leveraging the noise inherent in wireless communications.
% Wheras, [S40] presents a defense strategy for enhancing the robustness of automatic modulation classification (AMC) models against adversarial attacks and unknown signal conditions. The approach integrates Spatial Transformer Networks (STN) with a novel ResNeXt architecture, termed STN-ResNeXt, to autonomously learn spatial transformations and adapt to variations in signal and channel conditions. Additionally, transfer learning (TL) is employed to transfer learned features from known scenarios to related tasks with limited labeled data, improving model generalizability. Through extensive performance analysis, the proposed defense demonstrates significant improvements in classification accuracy across different channel conditions and signal parameters, highlighting the effectiveness of combining STN-based spatial transformation learning with TL for robust modulation classification.
% [S96] defense strategy introduces a machine unlearning method called detoxification to remove backdoors from neural network models without prior knowledge of the attack specifics. This method combines \emph{label smoothing} and \emph{adversarial training} in a minimax optimization framework to ensure the model accurately processes both clean and compromised inputs. It features a backdoor detection mechanism to assess model integrity. The core idea is to iteratively adjust the model to minimize the impact of adversarial perturbations, thereby eliminating the backdoor while preserving the model's performance on legitimate data. This approach not only neutralizes backdoor threats but also strengthens the model's overall security posture.
% Lastly, [S98] introduces a dynamic norm clipping technique alongside a federated noise titration scheme to detect and mitigate backdoor attacks in federated learning (FL) systems. The dynamic norm clipping approach adjusts the clipping threshold for model updates based on the server's analysis, which effectively prevents attackers from embedding backdoors into the global model without significantly affecting the performance of benign tasks. The federated noise titration scheme enhances detection capabilities by adding specific intensities of noise to user data and analyzing the model's response. This method leverages the observation that models compromised with backdoors respond differently to noisy inputs compared to benign models. By combining these two strategies, the defense aims to secure FL environments against backdoor threats while maintaining high accuracy for legitimate tasks, embodying a proactive and reactive defense mechanism
